Let Guidelines Guide You: A Prescriptive Guideline-Centered Data Annotation Methodology

We introduce the Guideline-Centered Annotation Methodology (GCAM), a novel data annotation methodology designed to report the annotation guidelines associated with each data sample. Our approach addresses three key limitations of the standard prescriptive annotation methodology by reducing the information loss during annotation and ensuring adherence to guidelines. Furthermore, GCAM enables the efficient reuse of annotated data across multiple tasks. We evaluate GCAM in two ways: (i) through a human annotation study and (ii) an experimental evaluation with several machine learning models. Our results highlight the advantages of GCAM from multiple perspectives, demonstrating its potential to improve annotation quality and error analysis.

==> src/background.tex <==

% \input{tables/glossary}

\section{Background and Motivation} \label{sec:background}


\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.8\columnwidth]{images/running_example.jpeg}
    \caption{\textbf{(a)} Example of guideline set $\mathcal{G}$ and class set $\mathcal{C}$ provided for annotation concerning hate speech detection. \textbf{(b)} In \stdabbrv, the annotator  is instructed with the mapping between $\mathcal{G}$ and $\mathcal{C}$ and associates data sample $x$ with the class subset $\mathcal{C}_x$ (blue box). \textbf{(c)} In \methodabbrv, the annotator is instructed with $\mathcal{G}$ only and defines a mapping between data sample $x$ and the guideline subset $\mathcal{G}_x$ (blue box). Subsequently, $x$ is associated with $\mathcal{C}_x$ thanks to a predefined mapping (green box).
    The example depicted is taken from \citet{kirk-et-al-2023-edos}.}
    \label{fig:running_example}
\end{figure*}

We formalize \stdabbrv to highlight its properties and limitations compared to \methodabbrv.
\Cref{tab:glossary} reports the notation used in the work to avoid potential ambiguity.
According to the prescriptive paradigm~\cite{rottger-etal-2022-two}, in \stdabbrv, a group of annotators labels data samples by following a set of detailed guidelines encoding the task. 
%
Standard practice typically dictates a preliminary stage both for annotators and guidelines: annotators should undergo a test to be assessed for eligibility~\cite{klie-etal-2024-dataset-annotation-quality}, and guidelines should be refined iteratively through one or multiple discussion phases on identified edge cases~\cite{caselli-etal-2020-feel, guzman-monteza-2023-annotation-method, jikeli-etal-2023-antisemitic-messages,kirk-et-al-2023-edos}.

%
In \stdabbrv, the labeling consists of mapping each data sample to one or more instances of the provided class set $\mathcal{C}$.
The class set $\mathcal{C}$ is task-specific and may vary according to the chosen problem formulation. 
%
Formally, given a dataset $\mathcal{X} = \{x_1, x_2, \dots, x_{\mid \mathcal{X} \mid}  \}$ and a class set $\mathcal{C} = \{c_1, c_2, \dots, c_{\mid \mathcal{C} \mid} \}$, annotators are asked to map a data sample $x \in \mathcal{X}$ to specific class subset $\mathcal{C}_x \subseteq \mathcal{C}$ by relying on the guideline set $\mathcal{G}= \{g_1, g_2, \dots, g_M \}.$\footnote{In a multi-class classification setting, the sample-specific class subset contains only one class (i.e., $\mathcal{C}_x = \{ c_x \}$).} The annotators are provided with the mapping between $\mathcal{G}$ and $\mathcal{C}$ to ground their annotations.
The annotation can be seen as a function that maps a data sample $x$ to its class subset $\mathcal{C}_x$:
 % 
\begin{equation} \label{eq:standard_}
    f: \mathcal{X} \rightarrow \mathcal{P}(\mathcal{C}),
\end{equation}

with $\mathcal{P}(\mathcal{C})$ the power set of the class set.
An example of \stdabbrv is depicted in \Cref{fig:running_example}(a,b), where the annotator implicitly uses the mapping between $\mathcal{G}$ and $\mathcal{C}$ to label $x$ as \texttt{sexist}.


%
% In \stdabbrv, annotators are not instructed to report the subset of guidelines they rely upon for annotating each data sample, which is lost at the end of the annotation process.
% We see this loss of information as a major drawback of the standard annotation process, potentially undermining the overall annotation quality. 
% In the remainder of the section, we discuss this aspect in detail, identifying three main critical issues.

\paragraph{Assumptions.}
%This work relies on the following assumptions.
For both \stdabbrv and \methodabbrv we assume that i)
the guideline set $\mathcal{G}$ is fixed throughout the data annotation process according to the prescriptive paradigm~\cite{rottger-etal-2022-two}, and ii)
data annotation guidelines can be framed as a set of criteria $g$.
%This is usually the case 
Criteria are used to reduce annotators' effort and provide systematic instructions that are easy to assimilate and follow~\cite{sabou-etal-2014-corpus, ruggeri-etal-2023-prescriptive-annotation}.

\subsection{Issues during Annotation Process} \label{sec:limitations:annot_process}
Evaluating annotation quality is crucial in ensuring the reliability of annotated data~\cite{klie-etal-2024-dataset-annotation-quality}.
The annotation quality can be influenced by three factors: i) intrinsic complexity of the task, ii) guidelines clarity and coverage of the task, and iii) annotators' understanding of the guidelines.
While task complexity is an inherent property of a problem, the other two factors can be addressed to enhance annotation quality.
%
In \stdabbrv, we do not have access to the guideline subset the annotators used for annotating each data sample. 
Therefore, verifying annotators' adherence to the guidelines is challenging. 
This has implications at two distinct stages. 
First, during the annotator eligibility assessment, it is difficult to determine whether they have assigned their labels following the provided guidelines or using their subjective criteria.
Second, during the annotation process, it is unclear whether errors stem from unclear guidelines or misinterpretation by the annotator. 

\subsection{Issues during Model Training}
\label{sec:limitations:model_training}
Machine Learning (ML) tasks are typically structured to enable a model to learn the relationship between input features ($x$) and target variables ($\mathcal{C}_x$).  
The underlying assumption is that the optimal mapping learned by the model from $x$ to $\mathcal{C}_x$ is the one adherent to the guideline set. 
However, no explicit constraints prevent the model from learning spurious correlations from data and, more in general, exploiting shortcuts~\cite{geirhos-et-al-2020-shortcut-learning}.
In principle, some models could potentially leverage the knowledge encoded in the guidelines subset $\mathcal{G}_x$ similarly to how external knowledge is integrated into machine learning models~\cite{von-rueden-etal-2023-informed-ml}. 
However, they need a dataset that contains this information to explicitly assess the knowledge integration process, which cannot be created with \stdabbrv.


==> src/discussion.tex <==
\section{Discussion} \label{sec:discussion}

\paragraph{Alternative Annotation Methodology.}
In \Cref{sec:gc:properties}, we discussed the benefits of the \methodabbrv methodology in reporting sample-specific guideline subset $\mathcal{G}_x$ compared to a standard annotation procedure.
As a possible alternative, we can consider an annotation process where the annotator reports \textit{both} the guideline subset $\mathcal{G}_x$ and the class subset $\mathcal{C}_x$ for each data sample.
This solution would allow for transparent adherence to annotation guidelines and fine-grained evaluation of annotations as \methodabbrv methodology.
However, this design choice is exposed to another form of annotation shortcut where the annotator may first determine $\mathcal{C}_x$ and then define $\mathcal{G}_x$ accordingly, thus reversing the expected annotation process.
Furthermore, as the standard annotation process, this alternative is tailored to a specific class set $\mathcal{C}$, implying that a change in $\mathcal{C}$ requires re-annotating collected data.
Lastly, reporting both $\mathcal{G}_x$ and $\mathcal{C}_x$ for a data sample $x$ carries the annotation cost of two distinct annotation processes, which is not desired.


\paragraph{Employing Fine-grained Class Sets.}
Another point of discussion concerns the use of a fine-grained class set $\mathcal{C}$ in place of the guideline set $\mathcal{G}$.
For instance, in~\citet{kirk-et-al-2023-edos}, the authors explore different class sets for hate speech detection, including one where each class $c$ has a one-to-one correspondence with a guideline definition $g$.
While an annotation process based on such a rich class set $\mathcal{C}$ allows for a fine-grained annotation evaluation, it still suffers from two main weaknesses: annotation 'shortcuts' and class set tight coupling.
First, an annotator might still leverage their own belief to align a data sample $x$ to a class $c$ while bypassing its corresponding guideline definition $g$.
As discussed in~\Cref{sec:background:limitations}, the risk that an annotator views a class $c$ and its corresponding guideline definition $g$ as two distinct concepts during annotation, thus, leading to shortcuts where $g$ is ignored, cannot be verified since the annotation process is adherent to the guideline set $\mathcal{G}$ only implicitly.
In contrast, in \methodabbrv, the annotation process is slightly different, where strict adherence to the guideline set $\mathcal{G}$ is the pivotal point of the annotation.
Thus, the risk of annotation 'shortcuts' is prevented.
Second, while a fine-grained class set allows for several potential class groundings to more coarse-grained class sets (e.g., class sets organized in a taxonomy as in~\citet{kirk-et-al-2023-edos}), it still limited in its flexibility in addressing different task formulations.
For instance, it is not possible to account for a change of the class grounding function $r$ while keeping the same class set $\mathcal{C}$ as in the subjectivity detection example discussed in~\Cref{sec:gc:properties}~\cite{antici-etal-2024-corpus-sentence}. 

\paragraph{Model Training with Guideline Definitions.}
In recent years, several works have highlighted the importance of leveraging the textual description corresponding to a class $c$ in addressing a text classification problem, whether in the form of class names, short descriptions, or task instructions.
These approaches differ in how class information is integrated and the particular learning method, whether through embedding-based enrichment~\cite{wang-etal-2018-joint-embedding,obeidat-etal-2019-description-typing,guo-etal-2021,ozmen-etal-2023-substituting,yin-etal-2023}, metric learning guidance~\cite{wohlwend-etal-2019,zhang-etal-2023-promptner,nghiem-etal-2024-define}, semantic retrieval~\cite{ruggeri-et-al-2022-tos,ruggeri-etal-2024-combining}, and by prompting LLMs~\cite{he-etal-2023-annollm,sainz-etal-2023-gollie,tan-etal-2024-data-annotation}, to name a few.
While these approaches demonstrate that integrating class textual descriptions achieves superior classification performance, they still rely on the class set $\mathcal{C}$ for model training supervision.
As discussed in~\Cref{sec:gc:properties}, this formulation suffers from unconstrained model training, where the adherence of the data-driven training approach to the task conveyed by the guideline set $\mathcal{G}$ is nuanced.
We argue that a shift towards training a model on predicting sample-specific guideline subsets $\mathcal{G}_x$ is needed to instruct and evaluate models in a way that is explicitly related to how a task is conceived, where an analysis through class symbols $c$ is always possible.
We leave the evaluation of data-driven models on reporting $\mathcal{G}_x$ as future work.



==> src/intro_old.tex <==
\section{Introduction}


High-quality data annotation requires clear guidelines. This is particularly true for subjective tasks such as hate speech detection~\cite{plank-etal-2014-linguistically,sap-etal-2022-annotators} and subjectivity detection~\cite{riloff-wiebe-2003-learning,savinova-moscoso-del-prado-2023-analyzing}.
Over the years, this has led to the development of various annotation paradigms. The most important paradigms are the prescriptive, descriptive, and perspectivist annotation paradigms.
The prescriptive annotation paradigm~\cite{rottger-etal-2022-two} enforces a shared belief of the task conveyed into a unique set of annotation guidelines on which annotators are instructed.
In contrast, the descriptive annotation paradigm~\cite{rottger-etal-2022-two} favors annotators' perspectives and beliefs, which are allowed to be reflected in the task.
In the perspectivist paradigm~\cite{cabitza-et-al-2023-perspectivist-turn}, multiple annotation ground truths for the same data sample are allowed while sharing a unique set of annotation guidelines.

All these paradigms follow a common approach. They define guidelines for annotators to associate classes with data samples.
Typically, the classes are defined based on a specific task, and the guidelines are only used for obtaining the class labels.
We argue that this annotation process has weaknesses that affect the quality of collected data and under-exploit annotators' potential contributions. 

In this paper, we expand on this concept by building on the prescriptive paradigm. 
The main idea is to define an annotation methodology that is focused on the guidelines by separating them from classes.
We call this novel methodology \method (\methodabbrv).
We discuss the advantages of \methodabbrv compared to existing methods and show experimentally that the approach is sustainable and can improve classification results.

\input{tables/glossary}

The remainder of this paper is structured as follows. In~\Cref{sec:background}, we discuss the standard annotation process under the prescriptive paradigm. Then, we 
introduce our methodology in~\Cref{sec:method}.
In~\Cref{sec:related} we frame our contribution with respect to the existing literature. 
Finally, we discuss some major implications of \methodabbrv in~\Cref{sec:discussion}, and report the concluding remarks in~\Cref{sec:conclusion}.




==> src/method.tex <==
\section{\methodabbrv} \label{sec:method}
%
We describe \method (\methodabbrv), a novel methodology aimed at enriching the annotation by keeping track of the guidelines associated with data samples. 
Conversely to \stdabbrv, in \methodabbrv, annotators do not have access to the class set, but only to the guidelines.
This ensures the annotation to be \textit{adherent to the guidelines} and  \textit{independent from the class set by definition}.

\subsection{Formalization} \label{sec:gc:formalization}
\methodabbrv comprises two stages. 
First, annotators are provided with guideline $\mathcal{G}$ and data $\mathcal{X}$, and are tasked with mapping each data point to their guideline subset $\mathcal{G}_x$. 
In the second phase, which does not involve annotators, one of the possible mappings between $\mathcal{G}$ and $\mathcal{C}$ is applied to associate samples to class labels.
%
Formally, \methodabbrv can be seen as the composition of two functions:
\begin{align}
    h &: \mathcal{X} \rightarrow \mathcal{P}(\mathcal{G}),
    \label{eq:two-stage_formulation_h}\\
    r &: \mathcal{G} \rightarrow \mathcal{C}.
    \label{eq:two-stage_formulation_r}
\end{align}
%
\Cref{eq:two-stage_formulation_h} represents the annotator's  function that maps a data sample $x$ to a guideline subset $\mathcal{G}_x$, while \Cref{eq:two-stage_formulation_r} is the \textit{class grounding function} mapping each guideline $g$ to the corresponding class.
The function $h$ is a black box proper of each annotator, similar to $f$ in \Cref{eq:standard_}, while the class grounding function $r$ is known by design.
\Cref{fig:running_example}(c) illustrates \methodabbrv.
In the first stage, the human annotator maps $x = \textit{"Women are pigs"}$ to $\mathcal{G}_x = \{ g_1 \}$.
Then, in the second stage, $\mathcal{G}_x$ is mapped to $\mathcal{C}_x = \{ \texttt{sexist} \}$ via $r$.



\subsection{Properties} \label{sec:gc:properties}
In the following, we describe four major properties of \methodabbrv addressing the issues of \stdabbrv (\S\ref{sec:background}).
\Cref{tab:method-summary} provides a summary.

\input{tables/method_summary}

\paragraph{Transparent Annotation Adherence to Guidelines.}

A key aspect of \methodabbrv is that annotators are unaware of the class set $\mathcal{C}$ and the class grounding function $r$.
This enforces adherence by definition to the guidelines during the annotation process, as the annotators do not have access to other information on the task.
In practice, \methodabbrv requires guidelines to not contain any reference to $\mathcal{C}$ and $r$.


\paragraph{Fine-grained Annotation Evaluation.}
Discussion phases are essential for the annotation procedure, as they serve the purpose of reaching an agreement on edge cases (\S\ref{sec:limitations:annot_process}).
In \methodabbrv, discussions revolve exclusively around the $\mathcal{G}_x$ and do not involve any reasoning on $\mathcal{C}$, as annotators lack access to it during the annotation phase. 
In this setting, the convergence of annotators' points of view can be effectively evaluated by inspecting $\mathcal{G}_x$.


\paragraph{Different Task Formulations.}
\methodabbrv enables using the annotated dataset for different task formulations that share the same guidelines. These formulations may stem from a taxonomy \cite{kirk-et-al-2023-edos} or account for discrepancies in how a task should be addressed, as it is often the case in subjective tasks like subjectivity detection~\citep{antici-etal-2024-corpus-sentence}.
In Figure~\ref{fig:class-groundings}, we show an example with three different class sets $ \mathcal{C}^\alpha, \mathcal{C}^\beta, \mathcal{C}^\gamma$  corresponding to three possible formulations of the hate speech detection task. A human annotator annotates the data sample $x$ with its guideline subset. The resulting $\mathcal{G}_x$ is mapped to the three class subsets by applying the class grounding function $r$ linking $\mathcal{G}$ to the corresponding class set.
As a result, we have three different class subsets
$\mathcal{C}_x^\alpha$, $\mathcal{C}_x^\beta$, and $\mathcal{C}_x^\gamma$ with a  single human annotation stage. 
This is a key advantage of \methodabbrv process over the \stdabbrv, in which changing the class set would require new annotation. 

\begin{figure}[!tb]
    \centering
    \includegraphics[width=\columnwidth]{images/class_groundings.jpeg}
    \caption{\methodabbrv allows defining different class sets ($\mathcal{C}^\alpha$, $\mathcal{C}^\beta$, $\mathcal{C}^\gamma$) and different class grounding functions ($r^\alpha$, $r^\beta$, $r^\gamma$) for the same guideline set $\mathcal{G}$ at the cost of a single human annotation stage (blue box).
    The annotator is unaware of the mapping between $\mathcal{G}$ and the class sets $\mathcal{C}^\alpha$, $\mathcal{C}^\beta$ and $\mathcal{C}^\gamma$ (green boxes).
    }
    \label{fig:class-groundings}
\end{figure} 




\paragraph{Model Training Advantages.}

Datasets created following \methodabbrv report explicitly the knowledge encoded in the guideline set $\mathcal{G}$.
% The \methodabbrv creates datasets containing the knowledge encoded in the guidelines subset \(\mathcal{G}_x\). 
This allows ML models to be effectively trained to leverage this information. 
%
% As pointed out in \Cref{sec:limitations:model_training}, the guideline set is not part of a standard ML model training procedure, causing a discrepancy between the human and the automated processes. 
% \methodabbrv provides datasets that would allow a supervised ML model to overcome this limitation by predicting $\mathcal{G}_x$ instead of $\mathcal{C}_x$.
% This training setting is consistent with the human annotation stage, as the ML model focuses on predicting the guideline subsets $\mathcal{G}_x$ provided by the annotators.
% We highlight three main advantages of supervising a model with $\mathcal{G}_x$ compared to $\mathcal{C}_x$.
We highlight three main advantages of training an ML model on \methodabbrv datasets.
First, we effectively prevent the model from learning spurious correlations between $x$ and $\mathcal{C}_x$, as the model has no access to $\mathcal{C}_x$ during training.
Second, the decoupling between $\mathcal{G}$ and $\mathcal{C}$ 
allows for using the ML model for different task formulations, as its predictions can be mapped to different class sets relying on the corresponding class grounding functions.
Third, we can evaluate the trained model's performance by assessing its alignment with the defined guidelines.
This involves analyzing disparities between predicted and ground-truth guideline subsets, fostering a deeper comprehension of the model's mechanisms.

%trained on a dataset $\mathcal{X}$ to class sets without the need for re-training it, as its predictions can be mapped to these class sets via their specific class grounding function $r$.
%allows using an ML model trained on a dataset $\mathcal{X}$ to class sets without the need for re-training it, as its predictions can be mapped to these class sets via their specific class grounding function $r$.

% A supervised model trained on a dataset annotated with \methodabbrv is consistent with the annotation process since it predicts the guideline subset $\mathcal{G}_x$ for each training sample $x \in \mathcal{X}$.
% Training the model to predict $\mathcal{G}_x$ has three main advantages.
% First, we effectively prevent it from learning spurious correlation between $\mathcal{X}$ and $\mathcal{C}$, as the model has no access to $\mathcal{C}_x$ during training.
% Second, the same trained model can be used for different task groundings without the need for retraining it, as its output can be mapped to different class sets depending on the defined class-specific function $r_G$.
% Third, the trained model's performance can be rigorously evaluated by assessing its alignment with defined guidelines.
% This assessment involves analyzing disparities between predicted and ground-truth guideline subsets, fostering a deeper comprehension of the model's  mechanisms.

% A dataset annotated with our \methodabbrv methodology can be used to train a supervised model to imitate the annotators' choice of guideline subsets. In particular,  the model is asked to predict the guideline subset $\mathcal{G}_x$ for each training sample $x \in \mathcal{X}$. 
% As the model has no access to $\mathcal{C}_x$ during training, we effectively prevent it from learning spurious correlation between $\mathcal{X}$ and $\mathcal{C}$. 
% Training the model to predict $\mathcal{G}_x$ has two main advantages. 
% First, once trained, the model can be used for different task groundings without the need for retraining it, as its output can be mapped to different class sets depending on the defined class-specific function $r_G$. 
% Second, the trained model's performance can be rigorously evaluated by assessing its alignment with defined guidelines. This assessment involves analyzing disparities between predicted and ground-truth guideline subsets, fostering a deeper comprehension of the model's  mechanisms.



%\TODO{We may remark that, in most of the cases, annotators' labels on the same data sample $x$ are aggregated. However, label aggregation is a process specific to certain annotation paradigms. This is just to say that there's always consistency.}




==> src/results.tex <==
\section{Results}
\TODO{Report results following the same order reported in Experiments section.}

\subsection{Annotation Study: Subjectivity Detection}

\subsection{Text Classification with Guidelines Only}

\input{tables/model_performance}
\subsubsection{Model Performance}

\subsubsection{Generalization to Unseen Labeling Criteria}

\subsection{Error Analysis with Guidelines}
One pivotal aspect of this study is the facilitation of error analysis through the use of guidelines. In this section, we examine the model errors and we attempt to delve further into the potential explanations by looking at the initial guidelines. In this way, we provide a comprehensive analysis that can highlight the model weaknesses on a semantic level. For our analysis, we look at the 4 best seeds of the models. or that reason, we divide our analysis into two parts. First, we compare the gold standard binary labels and the labels produced by the discreet model without considering the guidelines. Then, we compare the same labels, but also taking into consideration their corresponding guidelines. 

The results are presented in the form of a confusion matrix in Figure~\ref{fig:confusion_matrix_disecrete}

\begin{figure}
    \centering    \includegraphics[width = \linewidth]{images/confusion_matrix.pdf}
    \caption{Confusion matrix of predicted labels of the discrete model.}
    \label{fig:confusion_matrix_disecrete}
\end{figure}

The confusion matrix shows that the majority of the errors are false positives. To gain further insights about the types of the sentences that included errors, we proceed to sample 10 examples for each error group (FP, FN) and we perform a qualitative analysis. In the case of FN, although the language is not particularly vulgar, there are explicit indicators towards violence, or there are instances of sexism that has been normalized, such as mom jokes. In the case of FP, there were more ambiguous cases. 

As we mentioned, however, this analysis is based on samples. Reporting the guidelines allows a more thorough and informed evaluation that is not based on randomness. 

\begin{figure}
    \centering    \includegraphics[width = \columnwidth]{images/overlapping.pdf}
    \caption{Caption}
    \label{fig:overlapping}
\end{figure}

For example, when analyzing the results with the guidelines, we can instantly see the reason why there is possibly an error Figure~\ref{fig:overlapping}. 

\begin{figure}
    \centering    \includegraphics[width = \linewidth]{images/confusion_matrix_guidelines.pdf}
    \caption{Caption}
    \label{fig:confusion_matrix1}
\end{figure}


% BERIGHTBACK

% \subsection{LLMs prompting}



==> src/showcase.tex <==
% Re-write experiments.tex

==> tables/annotation_iaa.tex <==


\begin{table}[!t]
    \centering
    \begin{tabularx}{\columnwidth}{X|r|rr|r}
    \toprule
    & \multicolumn{1}{c|}{$p_{\stdabbrv}$} & \multicolumn{2}{c|}{$p_{\methodabbrv}$} & \multicolumn{1}{c}{\textit{All}} \\ 
    Batch & \multicolumn{1}{c|}{$\mathcal{C}_x$} & \multicolumn{1}{c}{$\mathcal{C}_x$} & \multicolumn{1}{c|}{$\mathcal{G}_x$} & \multicolumn{1}{c}{$\mathcal{C}_x$} \\ \midrule
    $b_1$ & 54.00 & 46.14 & 28.89 & 48.12 \\
    $b_2$ & 62.00 & 57.70 & 38.86 & 58.09 \\
    \bottomrule
    \end{tabularx}
    \caption{IAA on subjectivity detection case study. 
    % The \textit{Overall} column reports IAA when considering all pairs annotations.
    }
    \label{tab:annotation-case-study}
\end{table}

==> tables/cm_llms.tex <==

\begin{figure}[!t]
\small
\centering

% First Row (Two subtables side by side)
\begin{minipage}{0.4\linewidth}
\centering
\begin{subtable}[t]{1\textwidth}
\centering
\setlength{\arrayrulewidth}{0.3mm}
\setlength{\tabcolsep}{5pt} % Reduce padding to make tables smaller
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c}
% \hline
T / P & Neg. & Pos. \\
\hline
Neg. &  1647 &  338 \\
\hline
Pos. &  2 &  45 \\
% \hline
\end{tabular}
\caption{$\mathcal{C}_x$ for \stdabbrv} \label{fig:cm-llm-a}
\end{subtable}
\end{minipage}%
\hspace{2em}
\begin{minipage}{0.4\linewidth}
\centering
\begin{subtable}[t]{1\textwidth}
\centering
\setlength{\arrayrulewidth}{0.3mm}
\setlength{\tabcolsep}{5pt} % Reduce padding to make tables smaller
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c}
% \hline
T / P  & Neg. & Pos. \\
\hline
Neg. &  446 &  1539 \\
\hline
Pos. &  1 &  46 \\
% \hline
\end{tabular}
\caption{$\mathcal{C}_x$ for \methodabbrv} \label{fig:cm-llm-b}
\end{subtable}
\end{minipage}%

\caption{(a, b) Llama confusion matrices on ToS$_{LTD}$ for \stdabbrv and \methodabbrv, respectively.}\label{fig:cm-llm}
\end{figure}

==> tables/llm_prompts.tex <==
\begin{table}[!tb]
    \centering
    \footnotesize
    \begin{tabularx}{\columnwidth}{l|X}
    \toprule
        \bf Task & \bf Prompt \\ \midrule
        ToS$_{\stdabbrv}$ & You are an annotator for unfair clause detection in the legal domain concerning consumer contracts. 
        Your are given a guideline set about consumer contract unfairness for the user or client.
        Each guideline set item is described by an identifier and a definition.
        Read carefully the guideline set.
        Your task is to classify input text as an unfair clause for the user or client.
        Respond only yes or no. \\
        & Guidelines: \{\texttt{guidelines}\} \\
        & Text: \{\texttt{text}\} \\
        & Answer: \\ 
        \midrule
        ToS$_{\methodabbrv}$ & You are an annotator for unfair clause detection in the legal domain concerning consumer contracts. 
        Your are given a guideline set about consumer contract unfairness for the user or client.
        Each guideline set item is described by an identifier and a definition.
        Read carefully the guideline set.
        Your task is to assess if each guideline set item relates to the input text or not.
        Respond only by choosing from \{\texttt{guideline\_ids}\} or respond with NO if the guideline set does not relate to the input text. 
        Respond only yes or no. \\
        & Guidelines: \{\texttt{guidelines}\} \\
        & Text: \{\texttt{text}\} \\
        & Answer: \\  
        \midrule
        EDOS$_{\stdabbrv}$ & You are an annotator for sexism detection. You are given a guideline set about sexism detection. 
        Each guideline set item is described by an identifier and a definition. 
        Read carefully the guideline set. 
        Your task is to classify input text as containing sexism or not. 
        Respond only yes or no. \\
        & Guidelines: \{\texttt{guidelines}\} \\
        & Text: \{\texttt{text}\} \\
        & Answer: \\
        \midrule        
        EDOS$_{\methodabbrv}$ & You are an annotator for sexism detection. You are given a guideline set about sexism detection. 
        Each guideline set item is described by an identifier and a definition. 
        Read carefully the guideline set. 
        Your task is to assess if each guideline set item relates to the input text or not.
        Respond only by choosing from \{\texttt{guideline\_ids}\} or respond with no if the guideline set does not relate to the input text. 
        Respond only yes or no. \\
        & Guidelines: \{\texttt{guidelines}\} \\
        & Text: \{\texttt{text}\} \\
        & Answer: \\
        \bottomrule
    \end{tabularx}
    \caption{LLM prompts.}
    \label{tab:llm_prompts}
\end{table}

==> tables/method_summary.tex <==
\begin{table*}[!t]
    \centering
    \small

    \begingroup
    \renewcommand{\arraystretch}{1.2} % Default value: 1
    
    \begin{tabular}{p{\columnwidth}|p{\columnwidth}}
    \toprule
     \multicolumn{1}{c}{\bf Standard Annotation Methodology} & \multicolumn{1}{c}{\bf \method} \\ \midrule
     Human annotation by aligning data sample $x$ to $\mathcal{C}_x$ & Human annotation by aligning data sample $x$ to $\mathcal{G}_x$ \\
     % Annotation tailored to a specific $\mathcal{C}$ & Annotation agnostic of a specific $\mathcal{C}$ \\
     One-stage annotation: from $x$ to $\mathcal{C}_x$ & Two-stage annotation: from $x$ to $\mathcal{G}_x$ and to $\mathcal{C}_x$ \\
     % Cannot retrieve $\mathcal{G}_x$ from $\mathcal{C}_x$ & Can always retrieve $\mathcal{C}_x$ from $\mathcal{G}_x$ given $r$ \\
     Opaque human annotation adherence to $\mathcal{G}$ & Transparent human annotation adherence to $\mathcal{G}$  \\
     Coarse-grained evaluation based on $\mathcal{C}_x$ & Fine-grained evaluation based on $\mathcal{G}_x$ and $\mathcal{C}_x$ \\
     Inconsistency between annotation and model training & Consistency between annotation and model training \\
     Single task formulation (one class set) & Multiple task formulations (multiple class sets) \\
     \bottomrule
    \end{tabular}

    \endgroup
    
    \caption{Comparison between \stdabbrv and \methodabbrv.}
    \label{tab:method-summary}
\end{table*}


% \begin{table*}[!tb]
%     \centering
%     \small
%     \begin{tabular}{p{\columnwidth}|p{\columnwidth}}
%     \toprule
%     Standard & \method \\ \midrule
    % \multicolumn{2}{c}{Annotation} \\ \midrule  
    %  \begin{algorithmic}[1]
    %  \Procedure{Human Annotation}{}
    %     \State{\textbf{Require:} Dataset $\mathcal{X}$, Guideline set $\mathcal{G}$, Class set $\mathcal{C}$}
    %  \For{example $x \in \mathcal{X}$}
    %     \State{Define $\mathcal{C}_x$ via $f$}
    %     \State{Label $x$ with $\mathcal{C}_x$}
    %  \EndFor
    %  \State{\textbf{Output:} Dataset $\mathcal{X}_\mathcal{C} = \{(x_1, \mathcal{C}_{x_1}), \dots, (x_N, \mathcal{C}_{x_N}) \}$}
    %  \EndProcedure
    %  \end{algorithmic} &
    %  \begin{algorithmic}[1]
    %  \Procedure{Human Annotation}{}
    %     \State{\textbf{Require:} Dataset $\mathcal{X}$, Guideline set $\mathcal{G}$}
    %     \For{sample $x \in \mathcal{X}$}
    %         \State{Select $\mathcal{G}_x$ via $h_\mathcal{G}$}
    %         \State{Label $x$ with $\mathcal{G}_x$}
    %     \EndFor
    %     \State{\textbf{Output:} Dataset $\mathcal{X}_\mathcal{G} = \{(x_1, \mathcal{G}_{x_1}), \dots, (x_N, \mathcal{G}_{x_N}) \}$}
    %  \EndProcedure
    %  \vspace{0.1cm}
    %  \Procedure{Class Grounding}{}
    %     \State{\textbf{Require:} Dataset $\mathcal{X}_\mathcal{G}$, Class set $\mathcal{C}$, Class grounding function $r_\mathcal{G}$}
    %     \For{sample $(x, \mathcal{G}_x) \in \mathcal{X}_\mathcal{G}$}
    %         \State{$\mathcal{C}_x \gets \{r_\mathcal{G}(g) \, \vert \, g \in \mathcal{G}_x\}$}
    %         \State{Label $x$ with $\mathcal{C}_x$}
    %     \EndFor
    %     \State{\textbf{Output:} Dataset $\mathcal{X}_\mathcal{C} = \{(x_1, \mathcal{C}_{x_1}), \dots, (x_N, \mathcal{C}_{x_N}) \}$}
    %  \EndProcedure
    %  \end{algorithmic}
    %  \\ \midrule
    %  \multicolumn{2}{c}{Model Training} \\ \midrule
    %  Algo   &   Algo \\ \midrule
    %  \multicolumn{2}{c}{Comparison} \\ \midrule
%      Opaque adherence to $\mathcal{G}$ & Transparent adherence to $\mathcal{G}$  \\
%      Coarse-grained evaluation based on $\mathcal{C}_x$ & Fine-grained evaluation based on $\mathcal{G}_x$ \\
%      Annotation tailored to a specific $\mathcal{C}$ & Annotation independent of $r_\mathcal{G}$ \\
%      Inconsistency between annotation process and model training & Consistency between annotation process and model training \\
%      \bottomrule
%     \end{tabular}
%     \caption{Comparison between standard practice and our \method annotation process.}
%     \label{tab:method-summary}
% \end{table*}

==> tables/model_performance.tex <==
\begin{table*}[!tb]
\centering
% \footnotesize
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
                     & \multicolumn{2}{c}{ToS (A)} & \multicolumn{2}{c}{ToS (CH)} & \multicolumn{2}{c}{ToS (CR)} & \multicolumn{2}{c}{ToS (LTD)} & \multicolumn{2}{c}{ToS (TER)} & \multicolumn{2}{c}{EDOS} \\ \midrule
Model                & \multicolumn{1}{c}{$\mathcal{C}_x$}            & \multicolumn{1}{c}{$\mathcal{G}_x$}            & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}            & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}            & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}             & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}             & \multicolumn{1}{c}{$\mathcal{C}_x$}           & \multicolumn{1}{c}{$\mathcal{G}_x$}          \\ \midrule
Discrete             &  $43.93_{\pm 13.13}$            &    -          &   $76.41_{6.18}$            &  -            &   $58.60_{\pm 5.40}$           &   -           &   $53.60_{4.34}$            &   -             &      x.x         &        -       &      $73.42_{\pm 0.66}$       &    -        \\
Multi-label          &   $31.86_{\pm 7.85}$           &     $18.33_{\pm 5.22}$         &   $67.98_{5.59}$            &    $34.58_{4.61}$          &    $38.96_{\pm 9.91}$           &    $17.37_{\pm 3.59}$          &      $49.65_{\pm 3.28}$         &    $19.87_{2.70}$           &     x.x          &     x.x          &     $63.61_{\pm 2.41}$        &    $27.09_{\pm 2.69}$        \\
\methodabbrv w/ Dot &     x.x         &    x.x          &    $62.85_{7.95}$           &    $27.35_{2.94}$          &    $37.36_{\pm 9.95}$           &    $18.21_{\pm 3.24}$          &    $48.09_{5.48}$          &     $17.12_{2.70}$          &     x.x          &     x.x          &    $63.06_{\pm 1.90}$         &    $24.70_{\pm 2.07}$        \\
\methodabbrv w/ Concat    &    x.x          &    x.x          &    $72.63_{15.29}$           &   $18.02_{3.65}$           &     $46.57_{\pm 10.36}$          &    $19.46_{\pm 3.72}$          &     $52.04_{3.60}$          &    $20.31_{3.23}$           &       $46.57_{\pm 10.36}$        &     $19.46_{\pm 3.72}$          &    $66.70_{\pm 2.07}$         &   $18.19_{\pm 1.37}$         \\
\methodabbrv w/ Entail  &     x.x         &    x.x          &     $\mathbf{80.79_{3.61}}$          &    $\mathbf{44.92_{9.93}}$          &     $56.82_{\pm 7.35}$          &    $27.21_{\pm 5.36}$          &    $\mathbf{61.87_{2.68}}$           &     $\mathbf{21.49_{1.41}}$          &    x.x           &    x.x           &   $71.41_{\pm 2.35}$          &  $22.97_{\pm 3.14}$ \\ \bottomrule          
\end{tabular}%
}
\caption{TODO}
\label{tab:res:model-performance}
\end{table*}

==> tables/text_classication.tex <==

\begin{table*}[!tb]
\centering
% \footnotesize
\scriptsize
\begin{tabular}{ll|r|rrrr}
\toprule
{} & {} & \multicolumn{1}{c|}{\stdabbrv} & \multicolumn{4}{c}{\methodabbrv} \\
\noalign{\vskip -4pt} & & & & & & \\
\multicolumn{1}{c}{Dataset} & \multicolumn{1}{c|}{F$_1$} & \multicolumn{1}{c|}{\textit{Binary}} & \multicolumn{1}{c}{\textit{Fine-grained}} & \multicolumn{1}{c}{\textit{Dot}} & \multicolumn{1}{c}{\textit{Concat}} & \multicolumn{1}{c}{\textit{Entail}} \\ \midrule
\multirow{2}{*}{ToS$_{A}$}  & $\mathcal{C}_x$ & $71.61_{\pm 6.76}$ & $65.31_{\pm 4.15}$ & $67.07_{\pm 6.34}$ & $66.81_{\pm 6.78}$ & $\mathbf{80.14_{\pm 5.29}}$ \\
                          & $\mathcal{G}_x$ & -                  & $18.33_{\pm 5.22}$ & $18.31_{\pm 8.24}$ & $19.55_{\pm 7.44}$ & $\mathbf{37.49_{\pm 5.28}}$ \\
\noalign{\vskip -4pt} & & & & & & \\
\multirow{2}{*}{ToS$_{CH}$} & $\mathcal{C}_x$ & $87.96_{\pm 3.19}$ & $83.61_{\pm 2.90}$ & $80.93_{\pm 4.14}$ & $86.13_{\pm 7.70}$ & $\mathbf{90.23_{\pm 1.84}}$ \\
                          & $\mathcal{G}_x$ & -                  & $34.58_{\pm 4.61}$ & $27.35_{\pm 2.94}$ & $18.02_{\pm 3.65}$ & $\mathbf{44.92_{\pm 9.93}}$ \\
\noalign{\vskip -4pt} & & & & & & \\
\multirow{2}{*}{ToS$_{CR}$} & $\mathcal{C}_x$ & $\mathbf{79.02_{\pm 2.77}}$ & $38.96_{\pm 9.91}$ & $67.85_{\pm 5.33}$ & $72.72_{\pm 5.51}$ & $78.14_{\pm 3.76}$ \\
                          & $\mathcal{G}_x$ & -                  & $17.37_{\pm 3.59}$ & $18.21_{\pm 3.24}$ & $19.46_{\pm 3.72}$ & $\mathbf{27.21_{\pm 5.36}}$ \\
\noalign{\vskip -4pt} & & & & & & \\
\multirow{2}{*}{ToS$_{LTD}$} & $\mathcal{C}_x$ & $75.87_{\pm 2.36}$ & $73.70_{\pm 1.79}$ & $72.82_{\pm 3.04}$ & $75.00_{\pm 1.96}$ & $\mathbf{80.39_{\pm 1.40}}$ \\
                           & $\mathcal{G}_x$ & -                  & $19.87_{\pm 2.70}$ & $17.12_{\pm 2.70}$ & $20.31_{\pm 3.23}$ & $\mathbf{21.49_{\pm 1.41}}$ \\
\noalign{\vskip -4pt} & & & & & & \\
\multirow{2}{*}{ToS$_{TER}$} & $\mathcal{C}_x$ & $\mathbf{86.86_{\pm 1.54}}$ & $78.80_{\pm 5.56}$ & $80.44_{\pm 4.19}$ & $77.64_{\pm 4.81}$ & $84.57_{\pm 4.94}$ \\
                           & $\mathcal{G}_x$ & -                  & $10.16_{\pm 2.91}$ & $11.15_{\pm 1.50}$ & $10.38_{\pm 1.31}$ & $\mathbf{20.04_{\pm 3.08}}$ \\
\noalign{\vskip -4pt} & & & & & & \\
\multirow{2}{*}{EDOS}      & $\mathcal{C}_x$ & $\mathbf{81.74_{\pm 0.59}}$ & $71.67_{\pm 2.78}$ & $71.10_{\pm 2.20}$ & $74.96_{\pm 2.20}$ & $79.87_{\pm 2.24}$ \\
                           & $\mathcal{G}_x$ & -                  & $\mathbf{27.09_{\pm 2.69}}$ & $24.70_{\pm 2.07}$ & $18.19_{\pm 1.37}$ & $22.97_{\pm 3.14}$ \\ \bottomrule
\end{tabular}




\caption{Encoder-based model performance on ToS and EDOS datasets. Best results are in bold.}
\label{tab:experiments:encoder-based}
\end{table*}


==> tables/text_classification_llm.tex <==

\begin{table*}[!tb]
\centering
% \footnotesize
\scriptsize
\begin{tabular}{ll|rrr|rrr}
\toprule
{} & {} & \multicolumn{3}{c|}{\stdabbrv} & \multicolumn{3}{c}{\methodabbrv} \\
\noalign{\vskip -4pt} & & & & & & & \\
\multicolumn{1}{c}{Dataset} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{Mistral} & \multicolumn{1}{c}{Llama} & \multicolumn{1}{c|}{Phi} & \multicolumn{1}{c}{Mistral} & \multicolumn{1}{c}{Llama} & \multicolumn{1}{c}{Phi} \\ \midrule
\multirow{2}{*}{ToS$_{A}$}   & $\mathcal{C}_x$  & $57.07$ & $62.72$ & $\mathbf{64.10}$ & $0.59$ & $36.04$ & $37.80$ \\ 
                             & $\mathcal{G}_x$  & - & - & - & $0.11$ & $1.44$ & $\mathbf{3.89}$ \\
\noalign{\vskip -4pt} & & & & & & & \\
\multirow{2}{*}{ToS$_{CH}$}  & $\mathcal{C}_x$  & $\mathbf{62.43}$ & $60.80$ & $62.09$ & $1.70$ & $21.31$ & $8.35$ \\
                             & $\mathcal{G}_x$  & - & - & - & $0.08$ & $3.06$ & $\mathbf{2.16}$ \\
\noalign{\vskip -4pt} & & & & & & & \\
\multirow{2}{*}{ToS$_{CR}$}  & $\mathcal{C}_x$  & $55.76$ & $56.64$ & $\mathbf{59.96}$ & $2.46$ & $27.74$ & $25.23$ \\
                             & $\mathcal{G}_x$  & - & - & - & $0.46$ & $\mathbf{1.18}$ & $1.17$ \\
\noalign{\vskip -4pt} & & & & & & & \\
\multirow{2}{*}{ToS$_{LTD}$} & $\mathcal{C}_x$  & $\mathbf{60.71}$ & $55.79$ & $58.00$ & $8.74$ & $21.16$ & $7.87$ \\
                             & $\mathcal{G}_x$  & - & - & - & $0.57$ & $\mathbf{5.03}$ & $4.32$ \\
\noalign{\vskip -4pt} & & & & & & & \\
\multirow{2}{*}{ToS$_{TER}$} & $\mathcal{C}_x$  & $\mathbf{62.70}$ & $54.86$ & $57.81$ & $2.33$ & $18.21$ & $2.63$ \\
                             & $\mathcal{G}_x$  & - & - & - & $0.53$ & $0.99$ & $\mathbf{1.19}$ \\
\noalign{\vskip -4pt} & & & & & & & \\
\multirow{2}{*}{EDOS}        & $\mathcal{C}_x$  & $56.47$ & $\mathbf{67.93}$ & $63.47$ & $25.85$ & $38.80$ & $28.29$ \\
                             & $\mathcal{G}_x$  & - & - & - & $9.97$ & $\mathbf{11.27}$ & $5.02$ \\ \bottomrule
\end{tabular}

\caption{LLMs performance on ToS and EDOS datasets. Best results are in bold.}
\label{tab:experiments:llm-prompting}
\end{table*}


==> tables/text_classification_transposed.tex <==
\begin{table*}[!tb]
\centering
% \footnotesize
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
                     & \multicolumn{2}{c}{ToS (A)} & \multicolumn{2}{c}{ToS (CH)} & \multicolumn{2}{c}{ToS (CR)} & \multicolumn{2}{c}{ToS (LTD)} & \multicolumn{2}{c}{ToS (TER)} & \multicolumn{2}{c}{EDOS} \\ \midrule
Model                & \multicolumn{1}{c}{$\mathcal{C}_x$}            & \multicolumn{1}{c}{$\mathcal{G}_x$}            & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}            & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}            & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}             & \multicolumn{1}{c}{$\mathcal{C}_x$}             & \multicolumn{1}{c}{$\mathcal{G}_x$}             & \multicolumn{1}{c}{$\mathcal{C}_x$}           & \multicolumn{1}{c}{$\mathcal{G}_x$}          \\ \midrule
Discrete             &  $71.61_{\pm 6.76}$            &    -          &   $87.96_{\pm 3.19}$            &  -            &   $\mathbf{79.02_{\pm 2.77}}$           &   -           &   $75.87_{\pm 2.36}$            &   -             &      $\mathbf{86.86_{\pm 1.54}}$         &        -       &      $\mathbf{81.74_{\pm 0.59}}$       &    -        \\
Multi-label          &   $65.31_{\pm 4.15}$           &     $18.33_{\pm 5.22}$         &   $83.61_{\pm 2.90}$            &    $34.58_{\pm 4.61}$          &    $38.96_{\pm 9.91}$           &    $17.37_{\pm 3.59}$          &      $73.70_{\pm 1.79}$         &    $19.87_{\pm 2.70}$           &     $78.80_{\pm 5.56}$         &     $10.16_{\pm 2.91}$          &     $71.67_{\pm 2.78}$        &    $\mathbf{27.09_{\pm 2.69}}$        \\
\methodabbrv w/ Dot &     $67.07_{\pm 6.34}$         &    $18.31_{\pm 8.24}$          &    $80.93_{\pm 4.14}$           &    $27.35_{\pm 2.94}$          &    $67.85_{\pm 5.33}$           &    $18.21_{\pm 3.24}$          &    $72.82_{\pm 3.04}$          &     $17.12_{\pm 2.70}$         &     $80.44_{\pm 4.19}$          &     $11.15_{\pm 1.50}$         &    $71.10_{\pm 2.20}$         &    $24.70_{\pm 2.07}$        \\
\methodabbrv w/ Concat    &    $66.81_{\pm 6.78}$          &    $19.55_{\pm 7.44}$          &    $86.13_{\pm 7.70}$           &   $18.02_{\pm 3.65}$           &     $72.72_{\pm 5.51}$          &    $19.46_{\pm 3.72}$         &     $75.00_{\pm 1.96}$          &    $20.31_{\pm 3.23}$           &       $77.64_{\pm 4.81}$        &     $10.38_{\pm 1.31}$          &    $74.96_{\pm 2.20}$         &   $18.19_{\pm 1.37}$         \\
\methodabbrv w/ Entail  &      $\mathbf{80.14_{\pm 5.29}}$         &   $\mathbf{37.49_{\pm 5.28}}$         &     $\mathbf{90.23_{\pm 1.84}}$          &    $\mathbf{44.92_{\pm 9.93}}$          &     $78.14_{\pm 3.76}$          &    $\mathbf{27.21_{\pm 5.36}}$         &    $\mathbf{80.39_{\pm 1.40}}$           &     $\mathbf{21.49_{\pm 1.41}}$          &    $84.57_{\pm 4.94}$           &    $\mathbf{20.04_{\pm 3.08}}$           &   $79.87_{\pm 2.24}$          &  $22.97_{\pm 3.14}$ \\ \bottomrule          
\end{tabular}%
}
\caption{TODO}
\label{tab:experiments:text-classication}
\end{table*}

